Equipping Experts/Bandits with Long-term Memory

We propose the first reduction-based approach to obtaining long-term memory guarantees for online learning in the sense of Bousquet and Warmuth, 2002, by reducing the problem to achieving typical switching regret. Specifically, for the classical expert problem with $K$ actions and $T$ rounds, using our framework we develop various algorithms with a regret bound of order $\mathcal{O}(\sqrt{T(S\ln T + n \ln K)})$ compared to any sequence of experts with $S-1$ switches among $n \leq \min\{S, K\}$ distinct experts. In addition, by plugging specific adaptive algorithms into our framework we also achieve the best of both stochastic and adversarial environments simultaneously. This resolves an open problem of Warmuth and Koolen, 2014. Furthermore, we extend our results to the sparse multi-armed bandit setting and show both negative and positive results for long-term memory guarantees. As a side result, our lower bound also implies that sparse losses do not help improve the worst-case regret for contextual bandits, a sharp contrast with the non-contextual case.

==> conclusion.tex <==
\section{Conclusions}
xxx

% \paragraph{Acknowledgements.}
% The authors would like to thank Tim van Erven for introducing the problem and to thank
% Tim van Erven, Dirk van der Hoeven, and Wouter Koolen for helpful discussions throughout the projects, especially on the FTRL approach.
% The work was done while Kai Zheng visited the University of Southern California. Kai Zheng gratefully acknowledges financial support from China Scholarship Council.
